A Survey on Security and Privacy Issues of UAVs

In the 21st century, the industry of drones, also known as Unmanned Aerial Vehicles (UAVs), has witnessed a rapid increase with its large number of airspace users. The tremendous benefits of this technology in civilian applications such as hostage rescue and parcel delivery will integrate smart cities in the future. Nowadays, the affordability of commercial drones expands its usage at a large scale. However, the development of drone technology is associated with vulnerabilities and threats due to the lack of efficient security implementations. Moreover, the complexity of UAVs in software and hardware triggers potential security and privacy issues. Thus, posing significant challenges for the industry, academia, and governments. In this paper, we extensively survey the security and privacy issues of UAVs by providing a systematic classification at four levels: Hardware-level, Software-level, Communication-level, and Sensor-level. In particular, for each level, we thoroughly investigate (1) common vulnerabilities affecting UAVs for potential attacks from malicious actors, (2) existing threats that are jeopardizing the civilian application of UAVs, (3) active and passive attacks performed by the adversaries to compromise the security and privacy of UAVs, (4) possible countermeasures and mitigation techniques to protect UAVs from such malicious activities. In addition, we summarize the takeaways that highlight lessons learned about UAVs' security and privacy issues. Finally, we conclude our survey by presenting the critical pitfalls and suggesting promising future research directions for security and privacy of UAVs.

==> bibs/SecurityReferences.tex <==
\section*{Security and Privacy Related Papers found in the literature}
Among 130 papers found in the literature, we have selected relevant journal/conference papers published or under-review considering security and privacy concerns of MAVs/UAVs or surveying MAVs/UAVs challenges. 

\begin{itemize}
    \item The best related surveys found are:  \cite{Yaacoub2020}, \cite{Koubaa2019}, \cite{Nassi2019},\cite{Altawy2017} and \cite{Krishna2017}.

    \item The fist top security and privacy discussions found are: \cite{Nassi2019a}, \cite{Boroujerdian2018}, \cite{Young2016}, \cite{Lin2018}, \cite{Nassi2017} and \cite{Kwon2018}.   

    \item The second top S\&P discussions found are: \cite{Xiao2019}, \cite{Allouch2019}, \cite{Ward2017}, \cite{Petrovsky2015}, \cite{Rani2016}, \cite{Chang2017}, \cite{Choudhary2018}, \cite{Zhi2020}, \cite{Rivera2014}, \cite{Seo2016}, \cite{Maxa2017}, \cite{Sedjelmaci2016}, \cite{Edwin2016}, \cite{Yoon2017}, \cite{Bunse2018}, \cite{Sedjelmaci2018}, \cite{Watkins2018}, \cite{McCoy2019}, \cite{Fotouhi2019}, \cite{Cebeloglu2019} and \cite{Jamil2020},                    

    \item The third top S\&P discussions found are: \cite{Prapulla2017}, \cite{Rajatha2015}, \cite{Khan2020}, \cite{Dahiya2020}, \cite{Deebak2020}, \cite{Guo2020a} and \cite{Guo2020}.

\end{itemize}

Other relevant papers on UAVs: \cite{Boccadoro2020}, \cite{Hayat2016}, \cite{Shakhatreh2019}, \cite{Wang2020}, \cite{Hentati2020},   

















